Full Reciprocity-Gap Waveform Inversion in the frequency domain, enabling sparse-source acquisition

The quantitative reconstruction of sub-surface Earth properties from the propagation of waves follows an iterative minimization of a misfit functional. In marine seismic exploration, the observed data usually consist of measurements of the pressure field but dual-sensor devices also provide the normal velocity. Consequently, a reciprocity-based misfit functional is specifically designed, and defines the Full Reciprocity-gap Waveform Inversion (FRgWI ) method. This misfit functional provides additional features compared to the more traditional least-squares approaches with, in particular, that the observational and computational acquisitions can be different. Therefore, the positions and wavelets of the sources from which the measurements are acquired are not needed in the reconstruction procedure and, in fact, the numerical acquisition (for the simulations) can be arbitrarily chosen. Based on three-dimensional experiments, FRgWI is shown to behave better than Full Waveform Inversion (FWI) in the same context. Then, it allows for arbitrary numerical acquisitions in two ways: when few measurements are given, a dense numerical acquisition (compared to the observational one) can be used to compensate. On the other hand, with a dense observational acquisition, a sparse computational one is shown to be sufficient, for instance with multiple-point sources, hence reducing the numerical cost. FRgWI displays accurate reconstructions in both situations and appears more robust with respect to cross-talk than the least-squares shot-stacking.

==> utils_title-geophysics.tex <==
%\title{Full Reciprocity-Gap Waveform Inversion with arbitrary 
%       probing sources in the frequency domain}
\title{\update{
       Full Reciprocity-Gap Waveform Inversion, 
       % in the frequency domain, 
       enabling sparse-source acquisition}
       }
\renewcommand{\thefootnote}{\fnsymbol{footnote}} 

\author{Florian Faucher\footnotemark[1]\footnotemark[2], 
        Giovanni Alessandrini\footnotemark[3],
        H\'el\`ene Barucq\footnotemark[2], 
        Maarten V. de Hoop\footnotemark[4], 
        Romina Gaburro\footnotemark[5] and 
        Eva Sincich\footnotemark[3]}

\address{
\footnotemark[1]Faculty of Mathematics, 
                University of Vienna, 
                Oskar-Morgenstern-Platz 1, A-1090 Vienna, Austria.
                E-mail: \href{mailto:florian.faucher@univie.ac.at}
                             {\texttt{florian.faucher@univie.ac.at}}.  \\
\footnotemark[2]Inria Project-Team Magique-3D, E2S--UPPA, Pau, France.
                E-mail: \href{mailto:helene.barucq@inria.fr}{\texttt{helene.barucq@inria.fr}}. \\
\footnotemark[3]Dipartimento di Matematica e Geoscienze, 
                Universit\`{a} di Trieste, Italy,
                E-mails: \href{mailto:alessang@units.it}{\texttt{alessang@units.it}};
                         \href{mailto:esincich@units.it}{\texttt{esincich@units.it}}. \\ 
\footnotemark[4]Department of Computational and Applied 
                Mathematics and Department of Earth Science, 
                Rice University, Houston TX 77005, USA.
                E-mail: \href{mailto:mdehoop@rice.edu}{\texttt{mdehoop@rice.edu}}. \\
\footnotemark[5]Department of Mathematics and Statistics, 
                Health Research Institute (HRI), 
                University of Limerick, Ireland.
                E-mail: \href{mailto:romina.gaburro@ul.ie}{\texttt{romina.gaburro@ul.ie}}.
}

%% \footer{Example}
\lefthead{Faucher et al.}
\righthead{Full Reciprocity-gap Waveform Inversion}

